From Preferences to Prejudice: The Role of Alignment Tuning in Shaping Social Bias in Video Diffusion Models

Recent advances in video diffusion models have significantly enhanced text-to-video generation, particularly through alignment tuning using reward models trained on human preferences. While these methods improve visual quality, they can unintentionally encode and amplify social biases. To systematically trace how such biases evolve throughout the alignment pipeline, we introduce VideoBiasEval, a comprehensive diagnostic framework for evaluating social representation in video generation. Grounded in established social bias taxonomies, VideoBiasEval employs an event-based prompting strategy to disentangle semantic content (actions and contexts) from actor attributes (gender and ethnicity). It further introduces multi-granular metrics to evaluate (1) overall ethnicity bias, (2) gender bias conditioned on ethnicity, (3) distributional shifts in social attributes across model variants, and (4) the temporal persistence of bias within videos. Using this framework, we conduct the first end-to-end analysis connecting biases in human preference datasets, their amplification in reward models, and their propagation through alignment-tuned video diffusion models. Our results reveal that alignment tuning not only strengthens representational biases but also makes them temporally stable, producing smoother yet more stereotyped portrayals. These findings highlight the need for bias-aware evaluation and mitigation throughout the alignment process to ensure fair and socially responsible video generation.

==> tables/ethnicity_results.tex <==
\begin{table*}[h]
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{adjustbox}{max width=\textwidth}
{
\begin{tabular}{cccccc}
\toprule
\textbf{Model} & & \textbf{White} & \textbf{Black} & \textbf{Latino Hispanic} & \textbf{East Asian} \\
\midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Video\\Crafter\end{tabular}}} & Ratio & \underline{26.0}(W)/2.6/3.8/\textbf{54.4}(E)/2.6/5.0/5.8 & 19.6/\underline{19.0}(B)/4.2/\textbf{40.5}(E)/4.4/5.2/7.1 & 18.1/4.6/\underline{8.3}(L)/\textbf{54.6}(E)/5.2/5.4/4.0 & 17.3/3.0/4.2/\textbf{\underline{64.1}}(E)/5.8/3.8/2.0 \\
 & Entropy & 0.5257 & 0.6269 & 0.5457 & 0.3827 \\
 & Overall-C. & 0.3668 & 0.3859 & 0.3768 & 0.3324 \\
\midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}T2V\\Turbo\end{tabular}}} & Ratio & \underline{17.1}(W)/3.2/5.6/\textbf{47.4}(E)/12.5/13.1/1.2 & 13.9/\underline{14.1}(B)/8.5/\textbf{33.7}(E)/13.9/15.3/0.6 & 7.1/7.9/\underline{13.9}(L)/\textbf{34.1}(E)/22.2/14.3/0.4 & 7.5/2.6/8.7/\textbf{\underline{48.0}}(E)/21.2/11.9/0.0 \\
 & Entropy & 0.5614 & 0.6527 & 0.5575 & 0.4728 \\
 & Overall-C. & 0.3612 & 0.3635 & 0.3532 & 0.3629 \\
\toprule
 & & \textbf{Southeast Asian} & \textbf{Indian} & \textbf{Middle Eastern} & \textbf{Person} \\
\midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Video\\Crafter\end{tabular}}} & Ratio & 18.7/2.8/6.5/\textbf{59.5}(E)/\underline{5.8}(S)/3.8/3.0 & 17.7/12.3/8.5/\textbf{46.4}(E)/7.3/\underline{4.0}(I)/3.8 & 19.6/6.3/6.7/\textbf{55.6}(E)/2.4/4.8/\underline{4.6}(M) & 21.4/0.8/1.6/\textbf{\underline{64.3}}(E)/2.4/4.0/5.6 \\
 & Entropy & 0.3783 & 0.3824 & 0.3840 & 0.2740 \\
 & Overall-C. & 0.3433 & 0.3281 & 0.4940 & 0.3591 \\
\midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}T2V\\Turbo\end{tabular}}} & Ratio & 5.8/2.8/10.1/\textbf{42.9}(E)/\underline{25.8}(S)/12.7/0.0 & 8.7/9.9/9.5/\textbf{33.1}(E)/21.0/\underline{17.7}(I)/0.0 & 8.1/7.7/10.5/\textbf{41.1}(E)/18.5/13.3/\underline{0.8}(M) & 11.1/4.0/9.5/\textbf{\underline{36.5}}(E)/20.6/16.7/1.6 \\
 & Entropy & 0.4962 & 0.5394 & 0.5517 & 0.2817 \\
 & Overall-C. & 0.3597 & 0.3624 & 0.3641 & 0.3389 \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-4mm}
\caption{Ethnicity-centric evaluation on VideoCrafter and T2V-Turbo. Same ethnicity group ratios are \underline{highlighted} and higher ethnicity group ratios are \textbf{emphasized}.}
\vspace{-4mm}
\label{tab:ethnicity_results}
\end{table*}

==> tables/gender_ethn_results_lc.tex <==
\begin{table*}[h]
\centering
\small
\setlength{\tabcolsep}{2.5pt}
\begin{adjustbox}{max width=0.75\textwidth}
{
\begin{tabular}{ccccccccc}
\toprule
& Ethnicity & \textbf{White} & \textbf{Black} & \textbf{Latino} & \textbf{East Asian} & \textbf{Southeast Asian} & \textbf{Indian} & \textbf{Middle}  \\
\midrule
\midrule

\multirow{4}{*}{\textbf{VideoCrafter}} & Ratio (\underline{M}/W) & \underline{51.2}/48.8 & \underline{64.0}/36.0 & \underline{64.0}/36.0 & \underline{68.0}/32.0 & \underline{58.9}/41.1 & \underline{57.9}/42.1 & \underline{60.0}/40.0 \\
& ($\sigma$) & 5.1/7.0 & 6.2/6.7 & 6.2/6.7 & 6.8/7.9 & 5.9/7.8 & 1.1/3.3 & 3.3/2.3 \\
& Entropy & 0.4913 & 0.5644 & 0.6031 & 0.3958 & 0.5224 & 0.6390 & 0.5118  \\
& Overall-C. & 0.3619 & 0.3840 & 0.3754 & 0.3808 & 0.3765 & 0.3760 & 0.3822 \\

\midrule

\multirow{4}{*}{\textbf{T2V-Turbo}} & Ratio (M/\underline{W}) & 30.9/\underline{69.1} & 38.4/\underline{61.6} & 43.1/\underline{56.9} & 40.5/\underline{59.5} & 42.3/\underline{57.7} & 32.0/\underline{68.0} & 28.0/\underline{72.0} \\
& ($\sigma$) & 4.9/2.9 & 3.9/3.0 & 4.5/6.8 & 5.2/5.2 & 2.9/2.9 & 3.8/3.0 & 3.0/2.0 \\
& Entropy & 0.5471 & 0.6304 & 0.5458 & 0.3768 & 0.4551 & 0.5536 & 0.5803  \\
& Overall-C. & 0.3402 & 0.3597 & 0.3529 & 0.3609 & 0.3567 & 0.3593 & 0.3648 \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-2mm}
\caption{Gender-centric evaluation across various video generative models under the ``gender+ethnicity'' setting, where prompts include only the term ``person.'' Higher gender ratios are highlighted with \underline{underlines}.}
\vspace{-4mm}
\label{tab:gender_ethn_results_lc}
\end{table*}

==> tables/gender_only_results_lc.tex <==
\begin{table*}[h]
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{adjustbox}{max width=0.9\textwidth}
{
\begin{tabular}{cccccccccccc}
\toprule
& Gender & \textbf{Man} & \textbf{Woman} & \textbf{Person} & \textbf{Non-binary} & & Gender & \textbf{Man} & \textbf{Woman} & \textbf{Person} & \textbf{Non-binary} \\
\midrule
\midrule

% \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Fast\\ Hunyuan\end{tabular}}} &  Ratio (M/W) & 61.8/38.2 & 45.9/54.1 & 59.0/41.0 & 60.8/39.2 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\Scope\end{tabular}}} & Ratio (M/W) & 69.9/30.1 & 56.2/43.8 & 63.7/36.3 & 55.6/44.4 \\
% &($\sigma$) & 6.8/7.8 & 7.9/7.0 & 1.9/1.1 & 9.2/10.7 & &($\sigma$) & 15.7/16.5 & 3.0/4.9 & 6.8/7.0 & 11.6/10.7 \\
% & Entropy & 0.4128 & 0.4215 & 0.4382 & 0.3554 & & Entropy & 0.3029 & 0.3929 & 0.3367 & 0.3430 \\
% & Overall-C. & 0.3615 & 0.3631 & 0.3554 & 0.3445 & & Overall-C. & 0.3425 & 0.3505 & 0.3409 & 0.3411 \\


\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\Scope\end{tabular}}} & Ratio (M/W) & 69.9/30.1 & \textcolor{red}{56.2/43.8} & \textcolor{blue}{63.7/36.3} & 55.6/44.4 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Instruct\\Video\end{tabular}}} & Ratio (M/W) & 78.4/21.6 & \textcolor{red}{53.3/46.7} & \uwave{51.6/48.4} & 66.1/33.9 \\
& ($\sigma$) & 15.7/16.5 & 3.0/4.9 & 6.8/7.0 & 11.6/10.7 & & ($\sigma$) & 4.5/3.4 & 1.1/3.3 & 0.6/0.6 & 2.3/3.3 \\
& Entropy & 0.3029 & 0.3929 & 0.3367 & 0.3430 & & Entropy & \underline{0.2113} & 0.2924 & 0.2825 & 0.2694 \\
& Overall-C. & 0.3425 & 0.3505 & 0.3409 & 0.3411 & &  Overall-C. & 0.3343 & 0.3447 & 0.3390 & 0.3261 \\
% \cmidrule{3-7}
% \cmidrule{10-14}
% & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & Ratio (M/W) & 67.6/32.4 & 47.5/52.5 & 63.6/36.4 & 60.5/39.5 & & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & Ratio (M/W) & 69.4/30.6 & 57.6/42.4 & 67.4/32.6 & 64.3/35.7 \\
% & & ($\sigma$) & 3.4/2.1 & 7.3/7.4 & 5.8/6.0 & 5.3/4.5 &  &  & ($\sigma$) & 2.7/2.4 & 3.4/3.9 & 1.1/1.9 & 1.3/1.3 \\ &  & Entropy & 0.3747 & 0.4171 & 0.3795 & 0.3298 &  &  & Entropy  & 0.2599 & 0.2892 & 0.2544 & 0.2604 \\
% &  & Overall-C. & 0.3757 & 0.384  & 0.3725 & 0.3673  &  &  & Overall-C. & 0.3512 & 0.3584 & 0.3465 & 0.3456 \\
% \midrule
% \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}T2V-\\ Turbo\end{tabular}}} &  Ratio (M/W) & \textcolor{red}{42.7/57.3} & 17.7/82.3 & 37.7/62.3 & 22.4/77.6 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Video\\Crafter\end{tabular}}} &  Ratio (M/W) & 50.8/49.2 & 42.3/57.7 & 54.0/46.0 & 58.2/41.8 \\
% &($\sigma$) & 5.9/5.9 & 4.5/5.1 & 1.13/1.13 & 5.9/4.9 & &($\sigma$) & 2.3/3.3 & 2.3/2.2 & 4.0/5.8 & 4.0/6.0 \\
% & Entropy & 0.2868 & 0.2045 & 0.2817 & 0.2320 &  & Entropy & 0.3118 & 0.3578 & 0.2740 & 0.3200 \\
% & Overall-C. & 0.3394 & 0.3454 & 0.3389 & 0.3295 &  & Overall-C. & 0.3608 & 0.3637 & 0.3591 & 0.3502 \\

\midrule
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Video\\Crafter\end{tabular}}} &  Ratio (M/W) & 50.8/49.2 & 42.3/57.7 & \uwave{54.0/46.0} & 58.2/41.8 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}T2V-\\ Turbo\end{tabular}}} &  Ratio (M/W) & \textcolor{red}{42.7/57.3} & 17.7/82.3 & \textcolor{blue}{37.7/62.3} & 22.4/77.6 \\
&($\sigma$) & 2.3/3.3 & 2.3/2.2 & 4.0/5.8 & 4.0/6.0 & &($\sigma$) & 5.9/5.9 & 4.5/5.1 & 1.13/1.13 & 5.9/4.9 \\
& Entropy & 0.3118 & 0.3578 & \underline{0.2740} & 0.3200 &  & Entropy & 0.2868 & \underline{0.2045} & 0.2817 & \underline{0.2320} \\
& Overall-C. & \underline{0.3608} & \underline{0.3637} & \underline{0.3591} & \underline{0.3502} &  & Overall-C. & 0.3394 & 0.3454 & 0.3389 & 0.3295 \\

% \cmidrule{3-7}
% \cmidrule{10-14}
% & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & Ratio (M/W) & \textcolor{red}{36.5/63.5} & 19.0/81.0 & 36.4/63.6 & 33.7/66.3 & & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & Ratio (M/W) & 62.9/37.1 & 46.2/53.8 & 60.6/39.4 & 60.2/39.8 \\
% & & ($\sigma$) & 1.2/1.1 & 2.2/2.3 & 1.5/1.1 & 0.6/0.6 &  &  & ($\sigma$) & 1.0/0.9 & 1.2/1.8 & 1.4/1.0 & 1.6/1.7 \\ &  & Entropy & 0.2586 & 0.2132 & 0.2541 & 0.3368 &  &  & Entropy  & 0.2827 & 0.2675 & 0.2685 & 0.2592 \\
% &  & Overall-C. & 0.3602 & 0.3670  & 0.3564 & 0.3518 &  &  & Overall-C. & 0.3814 & 0.3883 & 0.3767 & 0.3718 \\
% \midrule
% \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Pyramid\\ Flow\end{tabular}}} & Ratio (M/W) & 74.0/26.0 & 34.5/65.5 & 68.3/31.7 & 64.5/35.5 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Open\\Sora\end{tabular}}} &  Ratio (M/W) & 75.6/24.3 & 23.7/72.7 & 55.9/44.1 & 54.8/45.2 \\
% & ($\sigma$) & 3.0/3.0 & 1.1/5.1 & 8.5/8.9 & 7.0/9.6 &  & ($\sigma$) & 0.0/0.0 & 0.0/1.1 & 0.0/2.9 & 0.0/0.0 \\
% & Entropy & 0.3569 & 0.4021 & 0.4193 & 0.4232 & & Entropy & 0.2964 & 0.2522 & 0.2599 & 0.2948 \\
% & Overall-C. & 0.3343 & 0.3324 & 0.3274 & 0.3307 &  & Overall-C. & 0.3507 & 0.3544 & 0.3419 & 0.3430 \\
% \cmidrule{3-7}
% \cmidrule{10-14}
% & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & Ratio (M/W) & 80.8/19.2 & 35.5/64.5 & 71.4/28.6 & 74.0/26.0 & & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & Ratio (M/W) & 73.2/26.8 & 37.1/62.9 & 65.9/34.1 & 68.8/31.2 \\
% & & ($\sigma$) & 0.3/0.3 & 1.5/1.3 & 1.3/1.3 & 3.8/4.1 &  &  & ($\sigma$) & 0.1/0.3 & 0.1/0.2 & 0.1/0.1 & 0.3/0.4 \\ &  & Entropy & 0.3223 & 0.4123 & 0.3899 & 0.3868 &  &  & Entropy  & 0.2245 & 0.2524 & 0.2340 & 0.2050 \\
% &  & Overall-C. & 0.3435 & 0.3467 & 0.3412 & 0.3418 & & & Overall-C. & 0.3661 & 0.3747 & 0.3591 & 0.3576 \\
% \midrule
% \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Fast\\ Hunyuan\end{tabular}}} &  Ratio (M/W) & 61.8/38.2 & 45.9/54.1 & 59.0/41.0 & 60.8/39.2 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\Scope\end{tabular}}} & Ratio (M/W) & 69.9/30.1 & 56.2/43.8 & 63.7/36.3 & 55.6/44.4 \\
% &($\sigma$) & 6.8/7.8 & 7.9/7.0 & 1.9/1.1 & 9.2/10.7 & &($\sigma$) & 15.7/16.5 & 3.0/4.9 & 6.8/7.0 & 11.6/10.7 \\
% & Entropy & 0.4128 & 0.4215 & 0.4382 & 0.3554 & & Entropy & 0.3029 & 0.3929 & 0.3367 & 0.3430 \\
% & Overall-C. & 0.3615 & 0.3631 & 0.3554 & 0.3445 & & Overall-C. & 0.3425 & 0.3505 & 0.3409 & 0.3411 \\
% \cmidrule{3-7}
% \cmidrule{10-14}
% & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & Ratio (M/W) & 67.6/32.4 & 47.5/52.5 & 63.6/36.4 & 60.5/39.5 & & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & Ratio (M/W) & 70.6/29.4 & 55.0/45.0 & 67.4/32.6 & 67.4/32.6 \\
% & & ($\sigma$) & 3.4/2.1 & 7.3/7.4 & 5.8/6.0 & 5.3/4.5 &  &  & ($\sigma$) & 4.1/3.5 & 7.1/6.8 & 2.3/2.9 & 4.6/4.3 \\ 
% & & Entropy & 0.3747 & 0.4171 & 0.3795 & 0.3298 & & & Entropy & 0.3084 & 0.3499 & 0.3100 & 0.3339 \\
% & & Overall-C. & 0.3757 & 0.384  & 0.3725 & 0.3673  & & & Overall-C. & 0.3543 & 0.3625 & 0.3507 & 0.3559 \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-2mm}
\caption{Gender-centric evaluation across different video generative models under ``gender-only'' setting. Higher overall consistency scores and lower entropy are \underline{highlighted}, while balanced ratios are \uwave{emphasized}.}
\vspace{-2mm}
\label{tab:gender_only_results_lc}
\end{table*}

==> tables/gender_results.tex <==
\begin{table*}[h]
\centering
\small
\setlength{\tabcolsep}{2.5pt}
\begin{adjustbox}{max width=0.85\textwidth}
{
\begin{tabular}{ccccccccc}
\toprule
\textbf{} & \textbf{Gender in Prompt} & \textbf{} & \multicolumn{3}{c}{\textbf{Man}} & \multicolumn{3}{c}{\textbf{Woman}} \\
\cmidrule{4-9}
\textbf{} & \textbf{Env. Setting} & \textbf{} & \textbf{HA} & \textbf{MA} & \textbf{LA} & \textbf{HA} & \textbf{MA} & \textbf{LA} \\
\midrule
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} \\
& & Entropy \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} \\
& & Entropy & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multirow{-6}{*}{\textbf{VADER}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. &  \\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} \\
& & Entropy \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. &\\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} \\
& & Entropy & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multirow{-6}{*}{\textbf{InstructVideo}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. &  \\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}75.0 / 25.0 \\ (1.96 / 2.99)\end{tabular} & \begin{tabular}[c]{@{}c@{}}60.3 / 39.7 \\ (2.96 / 3.39)\end{tabular} & \begin{tabular}[c]{@{}c@{}}64.0 / 36.0 \\ (2.99 / 3.88)\end{tabular} & \begin{tabular}[c]{@{}c@{}}13.0 / 87.0 \\ (2.99 / 2.26)\end{tabular} & \begin{tabular}[c]{@{}c@{}}18.5 / 81.5 \\ (6.84 / 7.84)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24.6 / 75.4 \\ (6.74 / 8.11)\end{tabular} \\
& & Entropy & 0.3597 & 0.4345 & 0.4253 & 0.3369 & 0.4625 & 0.4311 \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. & 0.3055 & 0.3370 & 0.3601 & 0.3086 & 0.3413 & 0.3623 \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}87.6 / 12.4 \\ (0.33 / 0.53)\end{tabular} & \begin{tabular}[c]{@{}c@{}}75.0 / 25.0 \\ (1.85 / 1.84)\end{tabular} & \begin{tabular}[c]{@{}c@{}}65.4 / 34.6 \\ (2.07 / 0.83)\end{tabular} & \begin{tabular}[c]{@{}c@{}}18.7 / 81.3 \\ (2.61 / 3.06)\end{tabular} & \begin{tabular}[c]{@{}c@{}}29.3 / 70.4 \\ (1.99 / 1.76)\end{tabular} & \begin{tabular}[c]{@{}c@{}}35.7 / 64.3 \\ (1.14 / 1.11)\end{tabular} \\
& & Entropy & 0.2764 & 0.3856 & 0.4182 & 0.3911 & 0.5002 & 0.4391 \\
\multirow{-6}{*}{\textbf{T2V-Turbo}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. & 0.3340 & 0.3661 & 0.3786 & 0.3391 & 0.3753 & 0.3877 \\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}} 99.2 / 0.8 \\ (2.26 / 1.13)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 85.4 / 14.6 \\ (1.92 / 1.96)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 74.0 / 26.0 \\ (2.99 / 2.99)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 9.8 / 90.2 \\ (1.96 / 2.99)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 28.3 / 71.7 \\ (2.99 / 1.08)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 34.5 / 65.6 \\ (1.08 / 5.14)\end{tabular}\\
& & Entropy & 0.1478 & 0.3258 & 0.3569 & 0.2957 & 0.4103 & 0.4021 \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. & 0.2801 & 0.3077 & 0.3343 & 0.2847 & 0.3082 & 0.3324 \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}} 92.0 / 8.0 \\ (0.41 / 0.60)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 92.2 / 7.8 \\ (0.91 / 1.40)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 80.8 / 19.2 \\ (0.33 / 0.28)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 17.6 / 82.4 \\ (1.57 / 1.00)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 29.8 / 70.2 \\ (1.79 / 1.85)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 35.5 / 64.5 \\ (1.47 / 1.27)\end{tabular}\\
& & Entropy & 0.1652 & 0.2526 & 0.3223 & 0.2679 & 0.3662 & 0.4123 \\
\multirow{-6}{*}{\textbf{Pyramid Flow}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. & 0.3026 & 0.3259 & 0.3435 & 0.3073 & 0.3310 & 0.3467 \\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}92.0 / 8.0 \\ (1.13 / 1.13)\end{tabular} & \begin{tabular}[c]{@{}c@{}}85.6 / 14.4 \\ (7.87 / 6.74)\end{tabular} & \begin{tabular}[c]{@{}c@{}}75.6 / 24.4 \\ (0 / 0)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24.4 / 75.6 \\ (1.13 / 1.96)\end{tabular} & \begin{tabular}[c]{@{}c@{}}33.1 / 66.9 \\ (4.48 / 4.03)\end{tabular} & \begin{tabular}[c]{@{}c@{}}27.3 / 72.7 \\ (0 / 1.13)\end{tabular} \\
& & Entropy & 0.3142 & 0.3599  & 0.3118 & 0.3408 & 0.3227 & 0.3578 \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. & 0.1887 & 0.2304 & 0.2964 & 0.2961 & 0.2250 & 0.2523 \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}88.6 / 11.4 \\ (0.29 / 0.61)\end{tabular} & \begin{tabular}[c]{@{}c@{}}90.6 / 9.4 \\ (0 / 0.14)\end{tabular} & \begin{tabular}[c]{@{}c@{}}73.2 / 26.8 \\ (0.14 / 0.33)\end{tabular} & \begin{tabular}[c]{@{}c@{}}15.6 / 84.4 \\ (0.24 / 0.28)\end{tabular} & \begin{tabular}[c]{@{}c@{}}23.4 / 76.6 \\ (0.33 / 0.66)\end{tabular} & \begin{tabular}[c]{@{}c@{}}37.1 / 62.9 \\ (0.14 / 0.19)\end{tabular} \\
& & Entropy & 0.0981 & 0.1050 & 0.2245 & 0.1857 & 0.2178 & 0.2524 \\
\multirow{-6}{*}{\textbf{Open-Sora}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. & 0.3280 & 0.3466 & 0.3661 & 0.3303 & 0.3547 & 0.3747  \\
\midrule

& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}70.6 / 29.4 \\ (5.95 / 5.95)\end{tabular} & \begin{tabular}[c]{@{}c@{}}68.3 / 31.7 \\ (8.49 / 10.09)\end{tabular} & \begin{tabular}[c]{@{}c@{}}50.8 / 49.2 \\ (2.26 / 3.35)\end{tabular} & \begin{tabular}[c]{@{}c@{}}22.6 / 77.4 \\ (4.03 / 3.39)\end{tabular} & \begin{tabular}[c]{@{}c@{}}40.3 / 59.7 \\ (7.37 / 6.25)\end{tabular} & \begin{tabular}[c]{@{}c@{}}42.3 / 57.7 \\ (2.26 / 2.22)\end{tabular} \\
& & Entropy & 0.3005 & 0.3231 & 0.3507 & 0.3042 & 0.3205 & 0.3544 \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. & 0.3156 & 0.3448 & 0.3608 & 0.3228 & 0.3493 & 0.3637 \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}78.2 / 21.8 \\ (1.93 / 1.60)\end{tabular} & \begin{tabular}[c]{@{}c@{}}73.0 / 27.0 \\ (0.99 / 0.14)\end{tabular} & \begin{tabular}[c]{@{}c@{}}62.9 / 37.1 \\ (1.01 / 0.91)\end{tabular} & \begin{tabular}[c]{@{}c@{}}33.5 / 66.4 \\ (0.80 / 0.94)\end{tabular} & \begin{tabular}[c]{@{}c@{}}45.0 / 55.0 \\ (1.74 / 1.13)\end{tabular} & \begin{tabular}[c]{@{}c@{}}46.2 / 53.8 \\ (1.25 / 1.80)\end{tabular} \\
& & Entropy & 0.2364 & 0.2711 & 0.2827 & 0.3212 & 0.2905 & 0.2675 \\
\multirow{-6}{*}{\textbf{VideoCrafter}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. & 0.3412 & 0.3716  & 0.3814 & 0.3637 & 0.3841 & 0.3883 \\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
& & Entropy & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
& & Entropy & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multirow{-6}{*}{\textbf{Hunyuan}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-2mm}
\caption{Gender-centric evaluation for subset ``Man'' and ``Woman''.}
\label{tab:gender_results_1}
\end{table*}

% Please add the following required packages to your document preamble:

% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\small
\setlength{\tabcolsep}{2.5pt}
\begin{adjustbox}{max width=0.85\textwidth}
{
\begin{tabular}{ccccccccc}
\toprule
\textbf{} & \textbf{Gender in Prompt} & \textbf{} & \multicolumn{3}{c}{\textbf{Person}} & \multicolumn{3}{c}{\textbf{No-Binary}} \\
\cmidrule{4-9}
\textbf{} & \textbf{Env. Setting} & \textbf{} & \textbf{HA} & \textbf{MA} & \textbf{LA} & \textbf{HA} & \textbf{MA} & \textbf{LA} \\
\midrule
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} \\
& & Entropy \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} \\
& & Entropy & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multirow{-6}{*}{\textbf{VADER}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. &  \\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} \\
& & Entropy \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. &\\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} \\
& & Entropy & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multirow{-6}{*}{\textbf{InstructVideo}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. &  \\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}71.9 / 28.1 \\ (3.35 / 2.99)\end{tabular} & \begin{tabular}[c]{@{}c@{}}57.6 / 42.4 \\ (3.88 / 4.03)\end{tabular} & \begin{tabular}[c]{@{}c@{}}63.2 / 36.8 \\ (5.61 / 4.89)\end{tabular} & \begin{tabular}[c]{@{}c@{}}65.8 / 34.2 \\ (2.99 / 2.22)\end{tabular} & \begin{tabular}[c]{@{}c@{}}54.6 / 45.4 \\ (4.89 / 3.35)\end{tabular} & \begin{tabular}[c]{@{}c@{}}54.0 / 46.0 \\ (10.70 / 11.83)\end{tabular} \\
& & Entropy & 0.5588 & 0.5045 & 0.4499 & 0.4776 & 0.5456 & 0.5127 \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. & 0.2965 & 0.3263 & 0.3471 & 0.2767 & 0.3166 & 0.3357 \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}86.9 / 13.1 \\ (0.74 / 1.07)\end{tabular} & \begin{tabular}[c]{@{}c@{}}70.7 / 29.3 \\ (1.11 / 0.70)\end{tabular} & \begin{tabular}[c]{@{}c@{}}61.2 / 38.8 \\ (0.88 / 0)\end{tabular} & \begin{tabular}[c]{@{}c@{}}82.0 / 18.0 \\ (0.28 / 0.70)\end{tabular} & \begin{tabular}[c]{@{}c@{}}70.0 / 3.0 \\ (1.16 / 1.32)\end{tabular} & \begin{tabular}[c]{@{}c@{}}58.6 / 41.4 \\ (2.90 / 1.84)\end{tabular} \\
& & Entropy & 0.3160 & 0.3999 & 0.4360 & 0.3664 & 0.4177 & 0.4229 \\
\multirow{-6}{*}{\textbf{T2V-Turbo}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. & 0.3232 & 0.3575  & 0.3697 & 0.3122 & 0.3436 & 0.3637 \\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}91.2 / 8.8 \\ (1.96 / 1.13)\end{tabular} & \begin{tabular}[c]{@{}c@{}}69.9 / 30.1 \\ (4.48 / 4.89)\end{tabular} & \begin{tabular}[c]{@{}c@{}}68.3 / 31.7 \\ (8.49 / 8.94)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}89.7 / 10.3 \\ (2.99 / 2.99)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}83.3 / 16.7 \\ (2.95 / 2.96)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}64.5 / 35.5 \\ (6.99 / 9.58)\end{tabular} \\
& & Entropy & 0.1811 & 0.3723 & 0.4193 & 0.2144 & 0.3289 & 0.4232 \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. & 0.2800 & 0.3033 & 0.3274 & 0.2735 & 0.3064 & 0.3307 \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}89.7 / 10.3 \\ (1.07 / 0.59)\end{tabular} & \begin{tabular}[c]{@{}c@{}}79.7 / 20.3 \\ (1.54 / 1.93)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}71.4 / 28.6 \\ (1.30 / 1.27)\end{tabular} & \begin{tabular}[c]{@{}c@{}}94.0 / 6.0 \\ (0.66 / 0.94)\end{tabular} & \begin{tabular}[c]{@{}c@{}}84.4 / 15.6 \\ (1.27 / 1.07)\end{tabular} & \begin{tabular}[c]{@{}c@{}}74.0 / 26.0 \\ (3.82 / 4.08)\end{tabular} \\
& & Entropy & 0.2210 & 0.3362 & 0.3899 & 0.1481 & 0.2892 & 0.3868 \\
\multirow{-6}{*}{\textbf{Pyramid Flow}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. & 0.2986 & 0.3257 & 0.3412 & 0.2923 & 0.3253 & 0.3418\\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}83.3 / 16.7 \\ (0 / 0)\end{tabular} & \begin{tabular}[c]{@{}c@{}}70.2 / 29.8 \\ (10.70 / 6.74)\end{tabular} & \begin{tabular}[c]{@{}c@{}}55.9 / 44.1 \\ (0 / 2.95)\end{tabular} & \begin{tabular}[c]{@{}c@{}}70.5 / 29.5 \\ (1.08 / 0)\end{tabular} & \begin{tabular}[c]{@{}c@{}}70.4 / 29.6 \\ (10.70 / 11.22)\end{tabular} & \begin{tabular}[c]{@{}c@{}}54.8 / 45.2 \\ (0 / 0)\end{tabular} \\
& & Entropy & 0.3639 & 0.3368 & 0.2741 & 0.3120 & 0.3047 & 0.3200 \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. & 0.3848 & 0.2256 & 0.2599 & 0.2300 & 0.2176 & 0.2948 \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}81.0 / 19.0 \\ (0.14 / 0.41)\end{tabular} & \begin{tabular}[c]{@{}c@{}}74.0 / 26.0 \\ (0.14 / 0.19)\end{tabular} & \begin{tabular}[c]{@{}c@{}}65.9 / 34.1 \\ (0.14 / 0.14)\end{tabular} & \begin{tabular}[c]{@{}c@{}}74.9 / 25.1 \\ (0.19 / 0.19)\end{tabular} & \begin{tabular}[c]{@{}c@{}}72.4 / 27.6 \\ (0.19 / 0.19)\end{tabular} & \begin{tabular}[c]{@{}c@{}}68.8 / 31.2 \\ (0.29 / 0.42)\end{tabular} \\
& & Entropy & 0.1524 & 0.1691 & 0.2340 & 0.1049 & 0.1459 & 0.2050 \\
\multirow{-6}{*}{\textbf{Open-Sora}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. & 0.3182 & 0.3408 & 0.3591 & 0.3169 & 0.3347 & 0.3576 \\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}70.5 / 29.5 \\ (7.88 / 5.15)\end{tabular} & \begin{tabular}[c]{@{}c@{}}60.8 / 39.2 \\ (5.61 / 5.61)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}54.0 / 46.0 \\ (4.05 / 5.84)\end{tabular} & \begin{tabular}[c]{@{}c@{}}72.4 / 27.6 \\ (6.25 / 6.25)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}61.1 / 38.9 \\ (4.48 / 4.48)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}58.2 / 41.8 \\ (4.03 / 6.99)\end{tabular} \\
& & Entropy & 0.2879 & 0.3142 & 0.3419 & 0.2933 & 0.3229 & 0.3430 \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. & 0.3092 & 0.3391 & 0.3591 & 0.2962 & 0.3294 & 0.3502 \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}77.8 / 22.2 \\ (1.13 / 0.47)\end{tabular} & \begin{tabular}[c]{@{}c@{}}67.1 / 32.9 \\ (2.07 / 2.07)\end{tabular} & \begin{tabular}[c]{@{}c@{}}60.6 / 39.4 \\ (1.43 / 1.01)\end{tabular} & \begin{tabular}[c]{@{}c@{}}73.2 / 26.8 \\ (0.14 / 0.14)\end{tabular} & \begin{tabular}[c]{@{}c@{}}64.2 / 35.8 \\ (2.73 / 2.88)\end{tabular} & \begin{tabular}[c]{@{}c@{}}60.2 / 39.8 \\ (1.57 / 1.67)\end{tabular} \\
& & Entropy & 0.2793 & 0.3030 & 0.2685 & 0.2284 & 0.2516 & 0.2592 \\
\multirow{-6}{*}{\textbf{VideoCrafter}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. & 0.3591 & 0.3699 & 0.3766 & 0.3502 & 0.3555 & 0.3718 \\
\midrule
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
& & Entropy & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ only\end{tabular}} & CLIP Con. & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\cmidrule{3-9}
& & \begin{tabular}[c]{@{}c@{}}Ratio \\ ($\sigma$) \end{tabular} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
& & Entropy & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multirow{-6}{*}{\textbf{Hunyuan}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Gender\\ +Ethnicity\end{tabular}} & CLIP Con. & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-2mm}
\caption{Gender-centric evaluation for subset ``Person'' and ``Non-binary Person''.}
\label{tab:gender_results_2}
\end{table*}

==> tables/hpdv2_gender_stats.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{adjustbox}{max width=\linewidth}
{
\begin{tabular}{ccccc}
\toprule
Dataset & \multicolumn{2}{c}{\textbf{Woman-Biased}} & \multicolumn{2}{c}{\textbf{Man-Biased}}  \\
\midrule
& \textbf{Ratio Diff.}  & \textbf{Count (M, W)} & \textbf{Ratio Diff.} & \textbf{Count (M, W)} \\
\midrule
\midrule
\multirow{10}{*}{\textbf{HPDv2}} & Bake: -1.0 & (0, 12) & Skate: 1.0 & (18, 0) \\ 
& Bike: -1.0 & (0, 6) & Row: 1.0 & (6, 0) \\ 
& Shop: -1.0 & (0, 6) & Drive: 1.0 & (270, 0) \\ 
& Shout: -1.0 & (0, 6) & Laugh: 0.75 & (210, 30) \\ 
& Cry: -0.673 & (48, 246) & Ride: 0.573 & (2694, 732) \\ 
& Pick: -0.667 & (48, 90) & Kneel: 0.563 & (150, 42) \\ 
& Smile: -0.612 & (192, 798) & Climb: 0.5 & (18, 6) \\ 
& Drink: -0.600 & (18, 72) & Jump: 0.4815 & (120, 48) \\
& Wash: -0.600 & (6, 24) & Throw: 0.340 & (42, 18) \\ 
& Paint: -0.582 & (114, 432) & Pray: 0.333 & (60, 30) \\ 
\midrule
\multirow{9}{*}{\textbf{PickaPic}} & Kneel: -1.0 & (0, 528) &  Lift: 1.0 & (13, 0) \\ 
& Shop: -1.0 & (0, 18) & Exercise: 1.0 & (3, 0) \\ 
& Shout: -1.0 & (0, 54) & Clean: 1.0 & (23, 0) \\ 
& Study: -1.0 & (0, 39) & Bake: 1.0 & (6, 0) \\ 
& Throw: -1.0 & (0, 54) & Laugh: 1.0 & (39, 17) \\ 
& Wash: -1.0 & (0, 27) &  \\ 
& Climb: -0.970 & (1, 66) & \\ 
& Jump: -0.748 & (13, 90) & \\
& Smile: -0.707 & (107, 624) & \\ 
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-4mm}
\caption{Top-k actions biased towards women and men.}
\label{tab:hpdv2_gender_results}
\vspace{-4mm}
\end{table}

==> tables/model_compare.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{adjustbox}{max width=0.75\linewidth}
{
\begin{tabular}{ccc}
\toprule
Model & \textbf{Reward Models} \\
\midrule
\midrule
%     &  & LAION aesthetic predictor V2~\citep{LAION-Aesthetics} \\
%                &  & HPSv2~\citep{wu2023human} \\
% \textbf{VADER}    & / & PickScore~\citep{Kirstain2023PickaPicAO} \\
%                &  & YOLOS~\citep{YOLOS} \\
%                &  & VideoMAE~\citep{tong2022videomae} \\
%                &  & V-JEPA~\citep{V-JEPA} \\
% \midrule
\textbf{InstructVideo} & HPSv2~\citep{wu2023human} \\
\midrule
& HPSv2.1~\citep{wu2023human} \\
\textbf{T2V-Turbo}  & InternVid2 S2~\citep{wang2024internvideo2} \\
& ViCLIP~\citep{wang2023internvid} \\
\midrule
\textbf{VideoCrafter} & / \\
\midrule
%                     & LAION-5B~\citep{laion-5b} &  \\
%                      & CC-12M~\citep{cc12m} &  \\
% \textbf{PyramidFlow}& Journey-DB~\citep{sun2023journeydb} & / \\
%                      & WebVid10M~\citep{bain2021frozen} &  \\
%                      & OpenVid-1M~\citep{OpenVid-1M} &  \\
%                      & 1M-Open-Sora Plan~\citep{open-sora-plan} &  \\
% \midrule
%                  & WebVid10M~\citep{bain2021frozen} &  \\
%                   & Panda-70M~\citep{Panda-70M} &  \\
%                   & HD-VG-130M~\citep{HD-VG-130M} &  \\
%                   & MiraData~\citep{MiraData} &  \\
%  \textbf{OpenSora} & Vript~\citep{yang2024vript} & / \\
%                   & Inter4K~\citep{Inter4K} &  \\
%                   & Unsplash-lite~\citep{unsplash} &  \\
%                   & LAION-5B~\citep{laion-5b} &  \\
%                   & Web-video from Pexels, Pixabay, and Mixkit &  \\
% \midrule
% \textbf{FastHunyuan} & NA & NA \\
% \midrule
\textbf{ModelScope} & / \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-2mm}
\caption{Comparison of different video generative models.}
\vspace{-2mm}
\label{tab:model_comparison}
\end{table}
















% \begin{table}[h]
% \centering
% \small
% \setlength{\tabcolsep}{2pt}
% \begin{adjustbox}{max width=\linewidth}
% {
% \begin{tabular}{ccc}
% \toprule
% Model & \textbf{Training Dataset} & \textbf{Reward Model} \\
% \midrule
% \midrule
% %     &  & LAION aesthetic predictor V2~\citep{LAION-Aesthetics} \\
% %                &  & HPSv2~\citep{wu2023human} \\
% % \textbf{VADER}    & / & PickScore~\citep{Kirstain2023PickaPicAO} \\
% %                &  & YOLOS~\citep{YOLOS} \\
% %                &  & VideoMAE~\citep{tong2022videomae} \\
% %                &  & V-JEPA~\citep{V-JEPA} \\
% % \midrule
% \textbf{InstructVideo} & WebVid10M~\citep{bain2021frozen} & HPSv2~\citep{wu2023human} \\
% \midrule
%              &  & HPSv2.1~\citep{wu2023human} \\
%  \textbf{T2V-Turbo}   & WebVid10M~\citep{bain2021frozen} & InternVid2 S2~\citep{wang2024internvideo2} \\
%                    &  & ViCLIP~\citep{wang2023internvid} \\
% \midrule
%                      & WebVid10M~\citep{bain2021frozen} &  \\
% \textbf{VideoCrafter} & JourneyDB~\citep{sun2023journeydb} & / \\
%                       & LAION-COCO~\citep{LAION-COCO} &  \\
% \midrule
% %                     & LAION-5B~\citep{laion-5b} &  \\
% %                      & CC-12M~\citep{cc12m} &  \\
% % \textbf{PyramidFlow}& Journey-DB~\citep{sun2023journeydb} & / \\
% %                      & WebVid10M~\citep{bain2021frozen} &  \\
% %                      & OpenVid-1M~\citep{OpenVid-1M} &  \\
% %                      & 1M-Open-Sora Plan~\citep{open-sora-plan} &  \\
% % \midrule
% %                  & WebVid10M~\citep{bain2021frozen} &  \\
% %                   & Panda-70M~\citep{Panda-70M} &  \\
% %                   & HD-VG-130M~\citep{HD-VG-130M} &  \\
% %                   & MiraData~\citep{MiraData} &  \\
% %  \textbf{OpenSora} & Vript~\citep{yang2024vript} & / \\
% %                   & Inter4K~\citep{Inter4K} &  \\
% %                   & Unsplash-lite~\citep{unsplash} &  \\
% %                   & LAION-5B~\citep{laion-5b} &  \\
% %                   & Web-video from Pexels, Pixabay, and Mixkit &  \\
% % \midrule
% % \textbf{FastHunyuan} & NA & NA \\
% % \midrule
%                 & WebVid10M~\citep{bain2021frozen} &  \\
% \textbf{ModelScope} & LAION-5B~\citep{laion-5b} & / \\
%                     & MSR-VTT~\citep{xu2016msr-vtt} &  \\
% \bottomrule
% \end{tabular}
% }
% \end{adjustbox}
% \vspace{-2mm}
% \caption{Comparison of different video generative models.}
% \label{tab:model_comparison}
% \end{table}


==> tables/models.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{adjustbox}{max width=0.9\linewidth}
{
\begin{tabular}{cc}
\toprule
Model & \textbf{Reward Models} \\
\midrule
\midrule
\textbf{ModelScope}    & HPSv2 \\
\textbf{InstructVideo} &  \\
\midrule
\textbf{Video-Crafter}& HPSv2.1 \\
\textbf{T2V-Turbo}     & InternVideo \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-2mm}
\caption{Comparison of model pairs and the used reward models.}
\label{tab:model-comparison}
\end{table}

==> tables/prompts_example.tex <==
\begin{wraptable}{r}{0.44\linewidth}
\vspace{-3mm}
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{adjustbox}{max width=\linewidth}
{
\begin{tabular}{m{2cm} m{3.8cm}}
\toprule
\multicolumn{1}{c}{\textbf{Bias}} & \multicolumn{1}{c}{\textbf{Examples}} \\
\midrule
Ethnicity Bias  & A \underline{person} is \textcolor{red}{\textbf{baking}} cookies in a cozy kitchen, with warm light and the aroma of vanilla filling the air. \\
\midrule
\makecell{Ethnicity-aware \\  Gender Bias} &  An \textcolor{blue}{\textit{East Asian}} \underline{person} is \textcolor{red}{\textbf{baking}} cookies in a cozy kitchen, with warm light and the aroma of vanilla filling the air. \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-2mm}
\caption{Prompts for Bias Evaluation: Each example highlights the actor's \underline{gender}, \textcolor{blue}{\textit{ethnicity}} (if specified), the \textcolor{red}{\textbf{action}}, and the surrounding context. 
%\junjie{the first row (Gender Only) doesn't specify a gender. you're still using "person".}
}
\vspace{-4mm}
\label{tab:prompts_stats}
\end{wraptable}


==> tables/reward_models_evaluation_apx.tex <==
% \vspace{-2mm}
\renewcommand{\arraystretch}{1.3}  % Increase row height
\begin{table}[h]
\centering
\setlength{\tabcolsep}{3pt}
\begin{adjustbox}{max width=\linewidth}
{
\begin{tabular}{ccccccccccccccccc}
\toprule
\textbf{Models} 
& \multicolumn{1}{c}{\textbf{Average}} 
& \multicolumn{2}{c}{\textbf{White}} 
& \multicolumn{2}{c}{\textbf{Black}} 
& \multicolumn{2}{c}{\textbf{Latino}} 
& \multicolumn{2}{c}{\textbf{East Asian}} 
& \multicolumn{2}{c}{\textbf{Southeast Asian}} 
& \multicolumn{2}{c}{\textbf{India}} 
& \multicolumn{2}{c}{\textbf{Middle Eastern}}
& \multicolumn{1}{c}{\textbf{Overall}} \\
\midrule
& \cellcolor{gray!7}PBS$_G$ & \cellcolor{gray!7}PBS$_G$ & RDS & \cellcolor{gray!7}PBS$_G$ & RDS & \cellcolor{gray!7}PBS$_G$ & RDS & \cellcolor{gray!7}PBS$_G$ & RDS & \cellcolor{gray!7}PBS$_G$ & RDS & \cellcolor{gray!7}PBS$_G$ & RDS & \cellcolor{gray!7}PBS$_G$ & RDS & SDI \\
\midrule
CLIP & \cellcolor{gray!7}-0.0726 & \cellcolor{gray!7}0.0343 & \textbf{\underline{0.0182}} & \cellcolor{gray!7}-0.1198 & 0.0002 & \cellcolor{gray!7}-0.0934 & -0.0013 & \cellcolor{gray!7}-0.1315 & 0.0141 & \cellcolor{gray!7}-0.0865 & 0.0094 & \cellcolor{gray!7}-0.0508 & -0.0299 & \cellcolor{gray!7}-0.0607 & -0.0108 & \textbf{\underline{0.8495}} \\
\cdashline{1-17} 
HPSv2.0 & \cellcolor{gray!7}0.6039 & \cellcolor{gray!7}0.6090 & -0.0423 & \cellcolor{gray!7}0.7341 & -0.0069 & \cellcolor{gray!7}0.6512 & 0.0237 & \cellcolor{gray!7}0.4752 & -0.0031 & \cellcolor{gray!7}0.5192 & -0.0100 & \cellcolor{gray!7}0.5922 & \underline{0.0070} & \cellcolor{gray!7}0.6464 & \textbf{\underline{0.0315}} & 0.8492 \\
$\Delta$ & \cellcolor{gray!7}\textcolor{red}{+0.6765} & \cellcolor{gray!7}\textcolor{red}{+0.5747} & \textcolor{orange}{-0.0605} & \cellcolor{gray!7}\textcolor{red}{+0.8539} & \textcolor{orange}{-0.0071} & \cellcolor{gray!7}\textcolor{red}{+0.7446} & \textcolor{teal}{+0.0250} & \cellcolor{gray!7}\textcolor{red}{+0.6067} & \textcolor{orange}{-0.0172} & \cellcolor{gray!7}\textcolor{red}{+0.6057} & \textcolor{orange}{-0.0194} & \cellcolor{gray!7}\textcolor{red}{+0.6430} & \textcolor{teal}{+0.0369} & \cellcolor{gray!7}\textcolor{red}{+0.7071} & \textcolor{teal}{+0.0423} & \textcolor{orange}{-0.0003} \\
\cdashline{1-17} 
HPSv2.1 & \cellcolor{gray!7}-0.0984 & \cellcolor{gray!7}-0.0833 & -0.0189 & \cellcolor{gray!7}0.0257 & -0.0321 & \cellcolor{gray!7}-0.0031 & \textbf{\underline{0.0382}} & \cellcolor{gray!7}-0.3044 & 0.0091 & \cellcolor{gray!7}-0.2181 & -0.0099 & \cellcolor{gray!7}-0.0006 & -0.0077 & \cellcolor{gray!7}-0.1053 & 0.0214 & 0.8470 \\
$\Delta$ & \cellcolor{gray!7}\textcolor{blue}{-0.0258} & \cellcolor{gray!7}\textcolor{blue}{-0.1176} & \textcolor{orange}{-0.0371} & \cellcolor{gray!7}\textcolor{red}{+0.1455} & \textcolor{orange}{-0.0323} & \cellcolor{gray!7}\textcolor{red}{+0.0903} & \textcolor{teal}{+0.0395} & \cellcolor{gray!7}\textcolor{blue}{-0.1729} & \textcolor{orange}{-0.0050} & \cellcolor{gray!7}\textcolor{blue}{-0.1316} & \textcolor{orange}{-0.0193} & \cellcolor{gray!7}\textcolor{red}{+0.0502} & \textcolor{teal}{+0.0222} & \cellcolor{gray!7}\textcolor{blue}{-0.0446} & \textcolor{teal}{+0.0322} & \textcolor{orange}{-0.0025} \\ 
\cdashline{1-17} 
PickScore & \cellcolor{gray!7}-0.1157 & \cellcolor{gray!7}0.0321 & 0.0069 & \cellcolor{gray!7}-0.0777 & \underline{0.0279} & \cellcolor{gray!7}-0.3479 & -0.0118 & \cellcolor{gray!7}-0.2257 & \textbf{\underline{0.0316}} & \cellcolor{gray!7}-0.2163 & \underline{0.0115} & \cellcolor{gray!7}0.1531 & -0.0391 & \cellcolor{gray!7}-0.1277 & -0.0271 & 0.8483 \\
$\Delta$ & \cellcolor{gray!7}\textcolor{blue}{-0.0431} & \cellcolor{gray!7}\textcolor{blue}{-0.0022} & \textcolor{orange}{-0.0113} & \cellcolor{gray!7}\textcolor{red}{+0.0421} & \textcolor{teal}{+0.0277} & \cellcolor{gray!7}\textcolor{blue}{-0.2545} & \textcolor{orange}{-0.0105} & \cellcolor{gray!7}\textcolor{blue}{-0.0942} & \textcolor{teal}{+0.0175} & \cellcolor{gray!7}\textcolor{blue}{-0.1298} & \textcolor{teal}{+0.0021} & \cellcolor{gray!7}\textcolor{red}{+0.2039} & \textcolor{orange}{-0.0092} & \cellcolor{gray!7}\textcolor{blue}{-0.0670} & \textcolor{orange}{-0.0163} & \textcolor{orange}{-0.0012} \\
\bottomrule
\end{tabular}
}
\end{adjustbox}
\vspace{-2mm}
\caption{Preference bias of different reward models. All values represent \textit{average} scores across 42 actions. 
% A positive PBS$_G$ score indicates a man-preference bias within the group, while a negative score reflects a woman-preference bias; values near zero suggest balanced gender representation. We annotate \textit{man-preferred} directions with (\textcolor{red}{+}) and \textit{woman-preferred} directions with (\textcolor{blue}{--}). A positive RDS$_e$ score signifies overrepresentation of a specific ethnicity group, while a negative score indicates underrepresentation; we highlight these with (\textcolor{teal}{+}) for \textit{overrepresentation} and (\textcolor{orange}{--}) for \textit{underrepresentation}. A higher SDI score denotes more balanced and diverse outputs across ethnic groups.
}
\label{tab:reward_model_evaluation_apx}
\end{table}

